Coping with Label Shift via Distributionally Robust Optimisation

The label shift problem refers to the supervised learning setting where the train and test label distributions do not match. Existing work addressing label shift usually assumes access to an \emph{unlabelled} test sample. This sample may be used to estimate the test label distribution, and to then train a suitably re-weighted classifier. While approaches using this idea have proven effective, their scope is limited as it is not always feasible to access the target domain; further, they require repeated retraining if the model is to be deployed in \emph{multiple} test environments. Can one instead learn a \emph{single} classifier that is robust to arbitrary label shifts from a broad family? In this paper, we answer this question by proposing a model that minimises an objective based on distributionally robust optimisation (DRO). We then design and analyse a gradient descent-proximal mirror ascent algorithm tailored for large-scale problems to optimise the proposed objective. %, and establish its convergence. Finally, through experiments on CIFAR-100 and ImageNet, we show that our technique can significantly improve performance over a number of baselines in settings where label shift is present.

==> rebuttal.tex <==

Reviewer 1:


-The improvement is either really limited on the test set by comparisons to the baseline (on Imagenet), or similar to that of the Agnostic method (on CIFAR-100, Appendix) 




More detailed explanation of the complexity of the algorithm in practice


More explanation on the choices of hyper-parameters


How/why do you choose these fixed values



Inner problem in (4) does indeed have a closed-form solution



Reviewer 3:


The DRO problem (3) and the mini batch gradient estimator are not new



Choosing the "right" value of gamma_c. 



We can also relax to the projection using KL-divergence to alleviate this difficulty.



Problem (3) and (4) are equivalent only if gamma_c is optimally tuned. 



Reviewer 4:


The argument that the authors make is that (b) is the important ingredient; that is, it is a question of optimization. Is this a fair characterization?



The authors write that the proximal mirror ascent updates solve the optimization instability (compared to the projection operator), but do not elaborate.



AdvShift is not optimizing properly with regard to the algorithm threshold r, as the authors point out. 



Sagawa et al. describe their method as using standard minibatching and SGD.



Is the pitch that one should use AdvShift when there are a large number of labels, but that it does not matter otherwise?

Why is there no difference in training error at tau = 0 even when training for a very conservative model (e.g., AdvShift 1.0, or Fixed 3)?  


The models used seem very underparameterized, presumably as a result of hyperparameter tuning; do they actually beat a normal ResNet with standard hyperparameters in the adversarial setting? 


Figs 2 and 3: Are the authors reporting test or validation accuracies? The figure captions all say validation, but the text all says test.



I am confused by why the fixed baseline does so badly. To clarify, for each value of tau, does each model have its own adversarial shift? Specifically, for the fixed model, is it still being evaluated against the fixed distribution? 


It is reasonable to focus on the adversarial setting, but the adversarial test error is still exceedingly high despite some improvements from AdvShift, so from the point of view of providing guarantees, this is only marginally better. 


If AdvShift helps on non-worst-case settings.






==> related.tex <==
We survey a number of related works.
Table~\ref{tbl:summary} summarises.

\begin{table}[!t]
    \centering
    \renewcommand{\arraystretch}{1.25}
    \begin{tabular}{@{}p{1.625in}p{3.5in}@{}}
        \toprule
        \textbf{Label distribution} & \textbf{Reference} \\
        \toprule
        Train distribution & Standard ERM \\
        Test distribution (estimated) & \citep{du2014semi,Lipton:2018,Azizzadenesheli:2018,Garg:2020,combes2020domain} \\
        Balanced & \citep{Xie:1989,Menon:2020} \\
        Worst class & \citep{Mohri:2019,Sagawa:2020} \\
        Worst $k$ classes & \citep{Williamson:2019,Curi:2019,Xu:2020} \\
        \midrule
        $f$-divergence ball around train distribution & This paper \\
        \bottomrule
    \end{tabular}
    \caption{Summary of existing approaches to learning with a modified label distribution.}
    \label{tbl:summary}
\end{table}

\subsection{Label shift and domain adaptation}
Most label shift works require having access to a fixed target distribution. \citep{Lipton:2018} shows that with access to a reasonable predictor and a unlabelled target distribution, one can estimate the label distribution using the predictor and get provable estimates on the label distribution in the target distribution. \citep{Azizzadenesheli:2018} relaxes the requirement on the predictor to allow confusion matrix have zero eigen gap by regularizing the label shift estimation. \citep{Garg:2020} solves the problem with an MLE approach and provide theoretical guarantee whent the predictor is calibrated. We emphasize that our approach differs from previous work in that we do not require access to sampling from the target distribution by learning an adversarial reweighting during training.

\cite{combes2020domain} talks about distribution shift in terms of label shift (different label distribution) instead of input shift. Hence, the work propose a domain adaptation algorithm that has the following component: 1. estimate an importance sampling weight on labels based on target distribution and source confusion matrix. 2. train a GAN model.

\cite{du2014semi} also considers the case when source and target has different label distributions. The algorithm first trains a standard classifier on the source distribution. Then use the source classifier to estimate distribution on target and reweight the loss in source.

The main difference in setting between our problem and domain adaptation is that we do not aim for best performance on a particular target distribution. Instead, we assume the target distribution is unknown, but close to the source.

\subsection{Distributionally robust optimisation}

\subsubsection{Generic uncertainty set}

\citet{Sagawa:2020}~considers the population as a mixture of subgroups. Then design a objective that minimizes the loss over all group instead of on the population.

\citet{Namkoong:2016}~considers a finite sum setting allow a perturbed distribution p around the uniform distribution over all samples. Since the problem is linear in p and convex in the argument, this is inherently a convex-concave problem. The main contribution is in generalization bound.

\citet{Sinha:2018}~considers min max problem, with nonconvex min (minimize neural net loss) and concave max (add strong regularizer to make the inner wasserstein robustness loss concave). Then convergence can be guaranteed. Certification part analyze generalization bound but is vacuous in real applications.

\citet{Namkoong:2017}~Robust regularized optimization (against $\chi^2$-divergence) is minimizing objective + variance under high probability.

\citet{Duchi:2018}~start the dual formulation robust optimization against perturbations measured by f-divergence. The problem  is convex. Hence the author uses interior point / GD with linesearch to solve the problem. More analysis on regret bound, consistency


\subsubsection{CVaR uncertainty set}

\citep{Rawat:2020} S2M algorithm (compute gradient using top k labels and top k samples) to highlight the weight of infrequent subpopulations. Theoretical connection to cvar.  Task: retrieval on Amazon-670k.


\citep{Curi:2019}~CVaR can be written as a maximization problem over distributions, which has a natural dual formulation. When the loss is convex, the minimization problem is convex and has subgradients. However, 1. Most gradients (except for alpha portion) is zero. 2. Rescaling makes gradient explode. Hence, formulate the problem as a min-max problem, where instead of uniform sampling the sampler consider the problem as a game and update weights using exp3. This is an interesting work, but is impractical in practice due the existence of kdpp and convex concave. 

\citep{Mohri:2019}~Projected gradient descent for both players. Optimization part. 

\citep{Xu:2020}~[this ties in to long-tail learning, since they mention using CVaR to account for label imbalance]

\citep{Li:2020} proposed a tilted empirical risk minimisation objective that interpolates between the minimum and maximum per-sample loss.


\subsubsection{Theoretical analysis for DRO against f-divergence}

Most theoretical work considers loss that is convex in model parameters. This way, even though the robust version is nonconvex, it is actually convex- concave, and its dual formulation can be solved by standard convex optimization. Some work also directly solves the min-max problem via primal-dual algorithms. We give a few examples below: \cite{fathony2018consistent}, this solves for a linear model by (1) fix the linear model, formulate the inner problem as linear programming, (2) solve the inner problem and evaluate gradient with respect to the model parameter. \cite{namkoong2017variance} solve the problem by solving the dual of inner problem, and evaluate the gradient.

\subsection{Long-tail learning}

\citep{Menon:2020} starts with the observation that known approaches (e.g. weight normalization, loss adjustment) are not consistent with the BER loss. Hence it proposes a consistent estimator by subtracting the log marginal probability from the logit. Test on artificial cifar, mnist dataset.

\citep{Cao:2019} Use hinge loss to maximize margin. Generalization bound with margin. Defer reeweighting. Artificially created cifar10 with long-tailed label distribution.

\citep{Kang:2020}








